Nonlinear System Identification of Soft Robot Dynamics Using Koopman Operator Theory

Soft robots are challenging to model due in large part to the nonlinear properties of soft materials. Fortunately, this softness makes it possible to safely observe their behavior under random control inputs, making them amenable to large-scale data collection and system identification. This paper implements and evaluates a system identification method based on Koopman operator theory in which models of nonlinear dynamical systems are constructed via linear regression of observed data by exploiting the fact that every nonlinear system has a linear representation in the infinite-dimensional space of real-valued functions called observables. The approach does not suffer from some of the shortcomings of other nonlinear system identification methods, which typically require the manual tuning of training parameters and have limited convergence guarantees. A dynamic model of a pneumatic soft robot arm is constructed via this method, and used to predict the behavior of the real system. The total normalized-root-mean-square error (NRMSE) of its predictions is lower than that of several other identified models including a neural network, NLARX, nonlinear Hammerstein-Wiener, and linear state space model.

==> outline.tex <==
\section{Outline}

\subsection{Introduction}
\subsection{Force Generation of Single Actuator}
\subsection{Force Generation of Parallel Combinations}
\subsection{Experiment/Model Validation}
\begin{itemize}
    \item Description of experimental setup (4 FREEs with orientation of end effector being measured)
    \item Math: How orientation is related to FREE states, q
    \item Sys ID for elastomer spring parameters
    \item Description of hardware, pictures, etc.
\end{itemize}
\subsection{Results}
Quantified error
\subsection{Discussion/Conclusion}
Sources of error: modeling assumptions and hardware
